Multilayer Perceptron Based Stress Evolution Analysis under DC Current Stressing for Multi-segment Wires

Electromigration (EM) is one of the major concerns in the reliability analysis of very large scale integration (VLSI) systems due to the continuous technology scaling. Accurately predicting the time-to-failure of integrated circuits (IC) becomes increasingly important for modern IC design. However, traditional methods are often not sufficiently accurate, leading to undesirable over-design especially in advanced technology nodes. In this paper, we propose an approach using multilayer perceptrons (MLP) to compute stress evolution in the interconnect trees during the void nucleation phase. The availability of a customized trial function for neural network training holds the promise of finding dynamic mesh-free stress evolution on complex interconnect trees under time-varying temperatures. Specifically, we formulate a new objective function considering the EM-induced coupled partial differential equations (PDEs), boundary conditions (BCs), and initial conditions to enforce the physics-based constraints in the spatial-temporal domain. The proposed model avoids meshing and reduces temporal iterations compared with conventional numerical approaches like FEM. Numerical results confirm its advantages on accuracy and computational performance.

==> bio.tex <==
\vspace{-10 mm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{tshou.jpg}}]
{Tianshu Hou} received the B.S. degree in electronic information science and technology from Sichuan University, Sichuan, China in 2019. She is currently pursuing a Ph.D degree in the Department of Micro/Nano-electronics, Shanghai Jiao Tong University, Shanghai, China. Her current research interests include electromigration reliability modeling, assessment and optimization.
\end{IEEEbiography}

\vspace{-15 mm}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{zpn.jpg}}]
{Peining Zhen}received the B.S. degree in electronic engineering from Sichuan University, Chengdu, China, in 2017. He is currently pursuing the Ph.D degree with the Department of Micro/Nano-Electronics, Shanghai Jiao Tong University, Shanghai, China. His current research interests include machine learning and neuromorphic computing.  
%is tensor-based computer vision methods.
\end{IEEEbiography}

\vspace{-15 mm}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{nwong.jpg}}]{Ngai Wong}  (SM, IEEE) received his B.Eng in 1999 and Ph.D. in EEE from The University of Hong Kong (HKU) in 2003, and he was a visiting scholar with Purdue University, West Lafayette, IN, in 2003. He is currently an Associate Professor with the Department of Electrical and Electronic Engineering at HKU. His research interests include electronic design automation (EDA), model order reduction, tensor algebra, linear and nonlinear modeling \& simulation, and compact neural network design. 
\end{IEEEbiography}

\vspace{-15 mm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{qchen.jpg}}]{Quan Chen} (S'09-M'11) received his B.S. degree in Electrical Engineering from the Sun Yat-Sen University, China, in 2005 and the M.Phil. and Ph.D. degree in Electronic Engineering from The University of Hong Kong, Hong Kong, in 2007 and 2010. From 2010-2011 he was postdoctoral fellow at the department of Computer Science and Engineering of the University of California, San Diego (UCSD). In 2012-2018, he was a research assistant professor at the department of Electrical and Electronic Engineering, The University of Hong Kong (HKU). He joined the Southern University of Science and Technology (SUSTech) in Shenzhen, China in 2019, where he is an assistant professor now. 
His research interests include ultra-large-scale circuit simulation and multi-physics analysis in the field of electronic design automation (EDA), as well as EDA techniques for emerging technologies such as sub-10nm devices, memristors, and quantum computing. He also has years of experience in technical transformation and commercialization.

\end{IEEEbiography}

\vspace{-15 mm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{GuoyongShi_pic.eps}}]{Guoyong Shi} (S'99-M'02-SM'11)
received the B.S. in applied mathematics from Fudan University, Shanghai, China, the M.S. degree in electronics and information science from Kyoto Institute of Technology, Kyoto, Japan, and the Ph.D. degree in electrical engineering from Washington State University, Pullman, in 1987, 1997, and 2002, respectively.

He is now a Professor of Microelectronics in Shanghai Jiao Tong University in Shanghai, China.
His research interests include design automation of analog/mixed-signal integrated circuits and systems.
He has published about 100 research papers in technical journals and conferences.
He is co-author of the book \emph{Advanced Symbolic Analysis for VLSI Systems --
Methods and Applications} published by Springer in 2014.
He has served several technical program committees including ASPDAC and SMACD.
He currently serves on the editorial board of Integration, the VLSI journal.
Dr. Shi was co-recipient of the Donald O. Pederson Best Paper Award in 2007.
\end{IEEEbiography}

\vspace{-10 mm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{sqwang.jpg}}]
{Shuqi Wang} received the B.Eng. degree in  Microelectronics Science and Engineering from University of Electronic Science and Technology of China, Sichuan, China in 2020. She is currently pursuing a master degree in the Department of Micro/Nano-electronics, Shanghai Jiao Tong University, Shanghai, China. Her research interests include machine learning and neuromorphic computing.
%machine learning in EDA and digital IC design.
\end{IEEEbiography}

\vspace{-15 mm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photo_hbchen.eps}}]
{Hai-Bao Chen} received the B.S. degree in information and computing sciences, and the M.S. and Ph.D. degrees in applied mathematics from Xian Jiaotong University, Xian, China, in 2006, 2008, and 2012, respectively. He then joined Huawei Technologies, where he focused on cloud computing and big data. He was a Post-Doctoral Research Fellow with Electrical Engineering Department, University of California, Riverside, CA, USA, from 2013 to 2014. He is currently an Associate Professor in the Department of Micro/Nano-electronics, Shanghai Jiao Tong University, Shanghai, China. His current research interests include VLSI reliability, machine learning and neuromorphic computing, numerical analysis and modeling for VLSIs, integrated circuit for signal and control systems. Dr. Chen has authored or co-authored about 70 papers in scientific journals and conference proceedings. He received one Best Paper Award nomination from Asia and South Pacific Design Automation Conference (ASP-DAC) in 2015. Since 2016, Dr. Chen serves as an Associate Editor for Integration-the VLSI Journal.
\end{IEEEbiography}





